Some Model Theory of Guarded Negation

The Guarded Negation Fragment (GNFO) is a fragment of first-order logic that contains all positive existential formulas, can express the first-order translations of basic modal logic and of many description logics, along with many sentences that arise in databases. It has been shown that the syntax of GNFO is restrictive enough so that computational problems such as validity and satisfiability are still decidable. This suggests that, in spite of its expressive power, GNFO formulas are amenable to novel optimizations. In this paper we study the model theory of GNFO formulas. Our results include effective preservation theorems for GNFO, effective Craig Interpolation and Beth Definability results, and the ability to express the certain answers of queries with respect to a large class of GNFO sentences within very restricted logics. This version of the paper contains streamlined and corrected versions of results concerning entailment of a conjunctive query from a set of ground facts and a theory consisting of GNFO sentences of a special form ("dependencies").

==> gnfokchar.tex <==

%PLACEHOLDER -- NEEDS TO BE REVISED

%\myparagraph{Characterizing $\gnfo^k$}
%We will now look at the corresponding expressive completeness result for $\gnfo^k$.
%In order to prove the Beth property of \gnfo (Theorem~\ref{thrm:Beth} below) 

\input{gnfokgame}
It is easy to see that $\gnfo^{k}$ formulas, and indeed even
$\gnfo^{+k}$ formulas, are preserved under such a game.
A characterisation stating that $\gnfo^k$ formulas are exactly
the first order formulas preserved by the Guarded Negation bisimulation game of
width $k$ was claimed in \cite{BtCS15jacm}.
We will prove a variation of this result, with one amendment and
two strengthenings. The amendment is that we claim that  $\gnfo^{+k}$ formulas
are exactly those preserved by the game, not only $\gnfo^k$ formulas.
%\begin{inparaenum} \item 
The first strengthening we require is that the formula be invariant only on models satisfying 
a given first-order sentence, while concluding that the formula is equivalent 
to a $\gnf^{+k}$ formula only for models of that sentence. Secondly, we show 
that if the formula is invariant when we look at $\gnkbisim$ equivalence 
in only a subset of the signature, then we can conclude that the formula is 
equivalent to a $\gnf^{+k}$ formula using only that subvocabulary.
This extension will be useful in our application to Beth
definability. 
%At the same time, we correct an error in the original argument
%from \cite{BtCS15jacm}.





Our next lemma states the game  characterizes $\gnfo^{+k}$-equivalence
assuming the models  are ``sufficiently rich''. 
We use $ \equiv_{\gnf^{k}[\tau]}$ to indicate that two structures with distinguished tuples
agree on all $\gnf^{k}$ formulas in signature $\tau$, and we use $\grd_\tau(\hat{\frakA})$ to indicate
the set of guarded tuples in structure $\hat{\frakA}$.
\begin{lemma}\label{lem:saturated}
  Consider $\omega$-saturated $\tau\cup\sigma$-structures $\tilde{\frakA}$ 
  and $\tilde{\frakB}$ and some $k>0$. Then the relation $Z_{k} = $
  $$
    \{ \, 
        (\bar{a},\bar{b}) \in \grd_\tau(\hat{\frakA}) \times \grd_\tau(\tilde{\frakB}) 
      \, \mid \, 
         \hat{\frakA},\bar{a} \equiv_{\gnf^{k}[\tau]} \tilde{\frakB},\bar{b}
      \, \}
  $$     
  is a GN-bisimulation of width $k$ between the $\tau$-reducts 
  of $\tilde{\frakA}$ and of $\tilde{\frakB}$.
\end{lemma}
\begin{proof}    
  Clearly, $Z_k$ consists of locally isomorphic pairs of tuples.
  We show that $Z_k$ satisfies the forth-clause, 
  the proof of the back-clause is analogous. 

  Suppose $(\bar c,\bar d)\in Z_k$ and let $X\subseteq \tilde{\frakA}$ with $|X|\leq k$.
  For simplicity, assume $\bar c\subseteq X$ (the general case is similar). 
  Thus, let $X=\{c_1,\cdots c_l,c_{l+1}, \ldots, c_n\}$ with $\bar c=(c_1,\cdots,c_l)$
  and $n\leq k$. Let $T[x_1, \ldots, x_n]$ be the set of all $\tau$-formulas 
  $\phi(x_1,\ldots, x_n)$ that are positive Boolean combinations of 
    (i) atomic $\tau$-formulas or 
   (ii) unary formulas of $\gnfo^k[\tau]$ or 
  (iii) formulas of the form $\gd_\tau(\bar y) \land \lnot\psi(\bar y) \in \gnfo^{+k}[\tau]$, 
  and that are true in $(\tilde{\frakA},c_1, \ldots, c_n)$. 
  We view $T$ as an $n$-type with $l$ parameters.  
  It is not hard to see that every finite subset $T'\subseteq T$ is realized in
  $\tilde{\frakB}$ under some assignment that sends $(x_1,\cdots,x_l)$ to $\bar d$.
  Indeed, notice that $\exists x_{l+1}\ldots x_n(\bigwedge T')$ is a formula 
  of $\gnfo^{+k}$ true at $\tilde{\frakA},\bar{c}$ and therefore it is also true 
  at $\tilde{\frakB},\bar{d}$.  
  Since $\tilde{\frakB}$ is $\omega$-saturated (and treating $T$ as an $n$-type
  with parameter $\bar{d}$) it follows that the entire set $T[x_1, \ldots, x_n]$ 
  is realized in $\tilde{\frakB}$ under an assignment $g$ 
  that sends $(x_1,\cdots,x_l)$ to $\bar{d}$.  
  It follows that $h:c_i \mapsto g(x_i)$ is a homomorphism such that, 
  for all $\bar{c'} \in \grd(\tilde{\frakA})$, i.e.,
  $\tilde{\frakA} \models \gd_\tau(\bar{c'})$ with $\bar{c'} \subseteq X$  
  we have $\tilde{\frakA},\bar{c'} \equiv_{\gnfo^{+k}[\tau]} \tilde{\frakB},h(\bar{c'})$ 
  and therefore $(\bar c',h(\bar c')) \in Z_k$ by definition of $Z_k$.
\end{proof}

We are now ready to prove  the corresponding semantic characterization of $\gnf^{+k}$:

\begin{theorem} \label{thrm_vanBenthem}
Let $\Phi$ be a set of $\fo[\tau\cup\sigma]$-sentences 
and $\varphi(\bar{x})$ an $\fo[\tau]$-formula that is $\gnkbisim$-invariant 
on the class of all $\tau$-reducts of $\Phi$-models and such that  all tuples
satisfying $\varphi(\bar{x})$ in models of $\Phi$ are $\tau$-guarded.
%the set of free variables of $\varphi(\bar{x})$ is guarded in $\tau$.
Then there exists a $\gnf^{+k}[\tau]$-formula $\vartheta(\bar{x})$ such that 
$\Phi \models \forall \bar{x} (\varphi(\bar{x}) \liff \vartheta(\bar{x}))$, with the equivalence
holding only on structures where the $\gd_\tau$ predicate is interpreted as the set of
$\tau$-guarded tuples.
\end{theorem}

In particular, the above implies that a first-order formula that is $\gnkbisim$-invariant
on all structures of a given signature is equivalent to a formula of $\gnf^{+k}$, where equivalence
enforces the ``built-in'' semantics of the $\gd_\tau$ predicate.


\begin{proof}
Consider 
$$
  \Psi = \{ \ \psi(\bar{x}) \in \gnf^{+k}[\tau] \ \mid \  
            \Phi, \varphi(\bar{x}) \models \psi(\bar{x}) \ \}  
$$ 
and assume that $\Psi\cup\Phi\cup\{\lnot\varphi(\bar{x})\}$ is satisfiable. 
%
Then there is some $\frakA \models \Phi$ and a tuple $\bar{a}$ in $\frakA$ 
such that $\frakA \models \psi(\bar{a}) \land \lnot\varphi(\bar{a})$ 
for all $\psi(\bar{x}) \in \Psi$. Let 
$$
  \Theta = \{ \ \vartheta(\bar{x}) \in \gnf^{+k}[\tau] \ \mid \
              \frakA \models \vartheta(\bar{a}) \ \} 
$$
and consider a model $\frakB \models \Phi$ and a tuple $\bar{b}$ in $\frakB$
such that $\frakB \models \vartheta(\bar{b})$ for all $\vartheta \in \Theta$. 
In other words, such that $\frakA,\bar{a} \equiv_{\gnf^k[\tau]} \frakB,\bar{b}$.
Let $\tilde{\frakA}$ and $\tilde{\frakB}$ be $\omega$-saturated elementary extensions 
of $\frakA$ and $\frakB$, respectively. 
In particular, $\tilde{\frakA}$ and $\tilde{\frakB}$ are models of $\Phi$. 
By Lemma~\ref{lem:saturated}, $\tilde{\frakA},\bar{a} \gnkbisim \tilde{\frakB},\bar{b}$ 
so by $\gnkbisim$-invariance of $\varphi$ on models of $\Phi$ we find that 
$\tilde{\frakB} \models \lnot\varphi(\bar{b})$ and therefore 
also $\frakB \models \lnot\varphi(\bar{b})$.
This shows that $\Theta\cup\Phi\cup\{\varphi(\bar{x})\}$ is unsatisfiable. 
By the Compactness Theorem for first order logic, there is a finite subset $\Theta_0 \subset \Theta$ such that 
$\Phi\cup\{\bigwedge\Theta_0(\bar{x}), \varphi(\bar{x})\}$ is unsatisfiable. 
Let $\vartheta(\bar{x}) = \gd_\tau(\bar{x}) \land \lnot \bigwedge\Theta_0(\bar{x})$, where
$\gd_\tau$ is a formula asserting that $\bar{x}$ is guarded by a $\tau$-atomic formula.
Keeping in mind the assumption on $\varphi(\bar{x})$,
%implies that the set of its free variables is guarded in $\tau$, 
we see that
$\Phi, \varphi(\bar{x}) \models \vartheta(\bar{x})$. 
But 
the conjunction with $\gd_\tau$ assures
that
$\vartheta(\bar{x}) \in \gnfo^{+k}[\tau]$; hence
$\vartheta(\bar{x}) \in \Psi \subset \Theta$ and thus $\frakA \models \vartheta(\bar{a})$ 
contradicting $\frakA \models \bigwedge\Theta_0(\bar{a})$.
 
It must therefore be the case that our initial assumption was false, 
so that $\Psi\cup\Phi\cup\{\lnot\varphi(\bar{x})\}$ is in fact unsatisfiable  
and, by compactness, that there exists a finite subset $\Psi_0 \subset \Psi$ 
such that $\Phi, \bigwedge\Psi_0(\bar{x}) \models \varphi(\bar{x})$. 
Note that also $\Phi, \varphi(\bar{x}) \models \bigwedge\Psi_0(\bar{x})$ so that 
$\Phi \models \forall \bar{x} ( \varphi(\bar{x}) \liff \bigwedge\Psi_0(\bar{x}))$.
In other words $\psi(\bar{x}) = \bigwedge\Psi_0(\bar{x}) \in \gnf^k[\tau]$ 
is equivalent to $\varphi(\bar{x})$ on all models of $\Phi$ as needed.
\end{proof}

Note that the  extension from $\gnf^k$ to $\gnf^{+k}$ is also needed to make the characterization theorem 
for $\gnkbisim$ stated in~\cite{BtCS15jacm} correct.





==> gnfokgame.tex <==
We now give the game associated
with the sublogic $\gnfo^k$ from ~\cite{BtCS15jacm}. We will show
that this game is actually ``exact'' for $\gnfo^{+k}$ formulas.
The guarded negation bisimulation game of width $k$
is an infinite game 
played on a pair of structures $\frakM,\frakN$ by two players: 
Mr.~Spoiler and Ms.~Duplicator. The game has two kinds of positions: 
\begin{compactitem}
  \item[i)] pairs of guarded tuples $(\bar{m},\bar{n})$, 
     such that $\bar{m}\mapsto\bar{n}$ is a partial isomorphism from $\frakM$ to $\frakN$; and 
 \item[ii)] partial homomorphisms $h:\frakM\restrict{}X \to \frakN\restrict{}Y$ or $g:\frakN\restrict{}Y \to \frakM\restrict{}X$, 
     where $X \subset \frakM$ and $Y \subset \frakN$, both finite  and $|X|,|Y| \leq k$.  
\end{compactitem}
From a position $(\bar{m},\bar{n})$ Spoiler must choose a finite subset $X \subset \frakM$ or 
a finite subset $Y \subset \frakN$ , in either case of size at most $k$, 
upon which Duplicator 
must respond by a homomorphism with domain $X$ or $Y$ accordingly, mapping it into the 
other structure in a manner consistent with $\bar{m}\mapsto\bar{n}$. 
From a position $h:X\to Y$ Spoiler chooses a guarded tuple $\bar{m}$ inside $X$ 
taking the play to the position $(\bar{m},h(\bar{m}))$. Similarly, from a position 
$g:Y \to X$ Spoiler chooses a guarded tuple $\bar{n}$ in $Y$ taking the play to the 
position $(g(\bar{n}),\bar{n})$. 
Spoiler wins if he can force the play into a position from which Duplicator cannot 
respond, and Duplicator wins if she can continue to play indefinitely. 
Two structures with initial tuples $\frakM,\bar{m}$ and $\frakN,\bar{n}$ are 
\emph{guarded negation bisimilar of width $k$}, 
in symbols $\frakM,\bar{m} \gnbisim^k \frakN,\bar{n}$,
if Duplicator has a winning strategy in the above game on $\frakM,\frakN$ from 
the initial position $(\bar{m},\bar{n})$. When the tuples
are empty, we talk about the two structures being GN-bisimilar of width $k$. Note that the tuples of the initial position 
need not be guarded, nor do they have to be of size at most $k$, 
but then a special rule 
must allow Spoiler to choose first, as the initial position for the $\gnbisim^k$-game as 
described above, a corresponding pair of sub-tuples $(\bar{m}^{\bar{\iota}},\bar{n}^{\bar{\iota}})$, 
such that at least one of them is guarded, and he immediately wins if only one of them 
is guarded, otherwise the game proceeds as above. \\



A \emph{rigid homomorphism} is a homomorphism $h: \frakM \to \frakN$ such that
 $\bar{m} \mapsto h(\bar{m})$ is a partial isomorphism for every guarded tuple $\bar{m}$
in the domain of $h$. Observe that in a GN-bisimulation game (of whatever width)
Duplicator must always play a (partial) rigid homomorphism in response to Spoiler's
every challenge to stay in the game.

 Guarded bisimilarity of width $k$ can be  reformulated in terms of the existence
of a certain kind of relation between tuples on the structures.
\begin{definition}[GN-bisimulations of width $k$]
  A GN-bisimulation of width $k$ between structures $\frakA$ and $\frakB$
  is a non-empty collection $Z$ of pairs $(\mathbf{a},\mathbf{b})$
  of guarded tuples of elements of $\frakA$ and of $\frakB$, respectively,
  such that for every $(\mathbf{a},\mathbf{b}) \in Z$:
  \begin{itemize}
  \item[(Forth)]
    for every $X\subseteq dom(\frakA)$ with $|X|\leq k$
    there is a partial homomorphism
    $h:\frakA \to \frakB$ with domain $X$ such that $h(a_i)=b_i$ for all $a_i\in X$ and
    such that ``$h$ is compatible with $Z$'', meaning that
    $(\mathbf{c},h(\mathbf{c}))\in Z$ for every guarded tuple $\mathbf{c}$ in $X$.
  \item[(Back)]
    for every $Y\subseteq dom(\frakB)$ with $|X|\leq k$
    there is a partial homomorphism
    $h:\frakB \to \frakA$ with domain $Y$ such that $h(b_i)=a_i$ for all $b_i\in Y$ and
    such that ``$h$ is compatible with $Z$'', meaning that
    $(h(\mathbf{c}),\mathbf{c})\in Z$ for every guarded tuple $\mathbf{c}$ in $Y$.
  \end{itemize}
  One can see that $(\frakA,\textbf{a})\sim^k_{gn} (\frakB,\textbf{b})$ holds exactly when
   $(\textbf{a},\textbf{b})$ belongs to a GN-bisimulation of width $k$  between $\frakA$ and $\frakB$

  As usual, this equivalence can  be indexed by a signature $\sigma$, in which case
  they are defined in terms of $\sigma$-reducts of the respective structures.
\end{definition}

\medskip









==> gnfpmacros.tex <==


%  ----------------------------------- M A C R O S --------------------------------

\newcommand{\locstruct}[1]{\ensuremath{\textup{LocStr}}(#1)}
\newcommand{\join}{\bowtie}

\newcommand{\myparagraph}[1]{{\bf {#1}.}}
\newcommand{\myeat}[1]{}
\newtheorem{theorem}{Theorem}[section]
%\newtheorem{metatheorem}{Metatheorem}[section]
%\newtheorem{example}[theorem]{Example}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proviso}[theorem]{Proviso}
\newtheorem{claim}[theorem]{Claim}


%\newcommand{\michael}[1]{{\bf Michael: #1}}
%\newcommand{\vince}[1]{{\bf Vince: #1}}
%\newcommand{\balder}[1]{{\bf Balder: #1}}

%LETTERS
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\frakd}{\mathfrak{d}}
\newcommand{\frakA}{\mathfrak{A}}
\newcommand{\frakB}{\mathfrak{B}}
\newcommand{\frakC}{\mathfrak{C}}
\newcommand{\frakD}{\mathfrak{D}}
\newcommand{\frakE}{\mathfrak{E}}
\newcommand{\frakF}{\mathfrak{F}}
\newcommand{\frakG}{\mathfrak{G}}
\newcommand{\frakH}{\mathfrak{H}}
\newcommand{\frakI}{\mathfrak{I}}
\newcommand{\frakJ}{\mathfrak{J}}
\newcommand{\frakK}{\mathfrak{K}}
\newcommand{\frakL}{\mathfrak{L}}
\newcommand{\frakM}{\mathfrak{M}}
\newcommand{\frakN}{\mathfrak{N}}
\newcommand{\frakO}{\mathfrak{O}}
\newcommand{\frakP}{\mathfrak{P}}
\newcommand{\frakQ}{\mathfrak{Q}}
\newcommand{\frakR}{\mathfrak{R}}
\newcommand{\frakS}{\mathfrak{S}}
\newcommand{\frakT}{\mathfrak{T}}
\newcommand{\frakU}{\mathfrak{U}}
\newcommand{\frakV}{\mathfrak{V}}
\newcommand{\frakW}{\mathfrak{W}}
\newcommand{\frakX}{\mathfrak{X}}
\newcommand{\frakY}{\mathfrak{Y}}
\newcommand{\frakZ}{\mathfrak{Z}}

\newcommand{\A}{{\mathcal A}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\C}{{\mathcal C}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\G}{{\mathcal G}}
\newcommand{\J}{{\mathcal J}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\Hch}{{\mathcal H}}
\newcommand{\T}{{\mathcal T}}
\newcommand{\Oh}{{\mathcal O}}
%\newcommand{\I}{{\mathcal I}} % conflict with already defined macro
\newcommand{\R}{{\mathcal R}}
\newcommand{\V}{{\mathcal V}}
\newcommand{\W}{{\mathcal W}}
\newcommand{\eS}{{\mathcal S}}


\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Int}{\mathbb{Z}}

\newcommand{\tup}[1]{{\bar {#1}}}
\newcommand{\tuple}[1]{{\bar {#1}}}


%%% LOGICAL SYMBOLS
\newcommand{\isom}{\cong}
\newcommand{\union}{\cup}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\limp}{\rightarrow}
\newcommand{\iffdef}{{\buildrel \rm def \over \iff}}
\newcommand{\eqdef}{{\buildrel \mathrm{def} \over =}}

%%% LOGICS, INTERPRETATIONS, QUANTIFIERS

\newcommand{\negNF}{negation normal form\xspace}
\newcommand{\gnnf}{GN-normal form\xspace}
\newcommand\mucalc{\ensuremath{\mu\text{-calculus}}\xspace}
\newcommand\fo{\ensuremath{\textup{FO}}\xspace}
\newcommand\mso{\ensuremath{\textup{MSO}}\xspace}
\newcommand\fp{\ensuremath{\textup{LFP}}\xspace}
\newcommand\gfo{\ensuremath{\textup{GFO}}\xspace}
\newcommand\founeg{\ensuremath{\textup{FO}(\neg_1)}\xspace}
\newcommand\fogneg{\ensuremath{\textup{GNFO}}\xspace}
\newcommand{\gnra}{\ensuremath{\textup{GN-RA}}\xspace}
\newcommand{\gf}{\gfo}
\newcommand\gnfo{\ensuremath{\textup{GNFO}}\xspace}
\newcommand\gnf{\gnfo}
\newcommand\gnfp{\ensuremath{\textup{GNFP}}\xspace}
\newcommand\gfp{\ensuremath{\textup{GFP}}\xspace}
\newcommand\unfo{\ensuremath{\textup{UNFO}}\xspace}
\newcommand\unfp{\ensuremath{\textup{UNFP}}\xspace}
\newcommand\fokneg{\ensuremath{\textup{FO}(\neg_k)}\xspace}
\newcommand\fpuneg{\ensuremath{\textup{MLFP}(\neg_1)}\xspace}
\newcommand\qbfuneg{\ensuremath{\textup{QBF}(\neg_1)}\xspace}
\newcommand\qbfkneg{\ensuremath{\textup{QBF}(\neg_k)}\xspace}
\newcommand\ctlx{\ensuremath{\textup{CTL}^*(\textsf{X})}\xspace}
\newcommand\ucq{\ensuremath{\textup{UCQ}}\xspace}
\newcommand\dnf{\ensuremath{\textup{DNF}}\xspace}
\newcommand{\gtgd}{\ensuremath{\textup{GTGD}}\xspace}
\newcommand{\fgtgd}{\ensuremath{\textup{FGTGD}}\xspace}
\newcommand{\tgd}{\ensuremath{\textup{TGD}}\xspace}



\newcommand{\complexity}[1]{\textsf{\mdseries\upshape #1}}
\newcommand\ptime{\textup{PTime}\xspace}
\newcommand\exptime{\textup{ExpTime}\xspace}
\newcommand\nexptime{\textup{NExpTime}\xspace}
\newcommand\twoexptime{\complexity{2ExpTime}}
%\newcommand\twoexptime{2{\sc ExpTime}\xspace}
\newcommand\np{\textup{NP}\xspace}
%\newcommand\conp{\textup{coNP}\xspace}
\newcommand\pnplog{\ensuremath{\textup{P}^{\textup{NP}[O(\log n)]}}\xspace}
\newcommand\pnplogsq{\ensuremath{\textup{P}^{\textup{NP}[O(\log^2 n)]}}\xspace}
\newcommand\pnp{\ensuremath{\textup{P}^{\textup{NP}}}\xspace}
\newcommand{\npnp}{\ensuremath{\textup{NP}^{\textup{NP}}}\xspace}
\newcommand{\conpnp}{\ensuremath{\textup{coNP}^{\textup{NP}}}\xspace}

\newcommand\grd{\ensuremath{\text{guarded}}}
\newcommand{\guarded}{\grd}
\newcommand\gd{\ensuremath{\mathsf{gd}}}
\newcommand{\gnbisimulation}[1]{\ensuremath{\sim_{gn[#1]}}}
\newcommand{\gnbisim}{\ensuremath{\sim_{gn}}}

\newcommand{\gnk}{\ensuremath{\mathrm{gn}[k]}\xspace}
\newcommand{\gnkbisim}{\sim^k_{gn}}

%\newcommand{\gnkbisim}{\ensuremath{\sim_{\gnk}}}

\newcommand{\restrict}{{\hskip-2pt}\upharpoonright{\hskip-3pt}}

\newcommand{\gnfoinference}{\hspace{.15em}\Rrightarrow_{\gnfo[\tau\cap\sigma]}\hspace{.15em}}
\newcommand{\gnfoequivalence}{\hspace{.15em}\equiv_{\gnfo[\tau\cap\sigma]}\hspace{.15em}}
	
%\newcommand{\twinshg}{{\hspace{.25em}{}^h\hspace{-.25em}\rightleftarrows_g\hspace{3pt}}}
%\newcommand{\twinsCPhg}{{\frakC \twinshg \frakP}}
%\newcommand{\twins}{\twinsCPhg}

\makeatletter
\def\@begintheorem#1#2{%
    \vspace{-3pt}
    \parskip -1pt % GM July 2000 (for tighter spacing)
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {{\sc #1}\hskip 5\p@\relax#2.}%
    ]
    \it
}
\let\old@endtheorem\@endtheorem
\def\@endtheorem{\old@endtheorem\vspace{-7pt}}
\makeatother
             






